Generalised Dining Philosophers as Feedback Control

We revisit the Generalised Dining Philosophers problem through the perspective of feedback control. The result is a modular development of the solution using the notions of system and system composition (the latter due to Tabuada) in a formal setting that employs simple equational reasoning. The modular approach separates the solution architecture from the algorithmic minutiae and has the benefit of simplifying the design and correctness proofs. Three variants of the problem are considered: N=1, and N>1 with centralised and distributed topology. The base case (N=1) reveals important insights into the problem specification and the architecture of the solution. In each case, solving the Generalised Dining Philosophers reduces to designing an appropriate feedback controller.

==> makefile <==
# This makefile can only be run from the command line
# after setting the following variable
# export TEXINPUTS=:lib/macros
FILE=dp
REP=tech-report
LATEX=pdflatex
TEXSTYLES=acmconf
# TEXPACKAGES=packages
# BSTINPUTS=:.:${TEXSTYLES}/IEEEtranBST//:
#BIBINPUTS=:.:biblio//:
#TEXINPUTS=${TEXSTYLES}//:${TEXPACKAGES}//:.:
TEXINPUTS=${TEXSTYLES}//:.:


# The paper includes a table summarising different approaches
# (See in the \include{approach-bib-stub} statement lit.tex.)
# First generate approach-bib.tex  from approach-bib.org
# Then grab the lines between \begin{center} and \end{center}
# and redirect to approach-bib-stub.tex, overwriting if necessary
# (hence, >|)

# https://stackoverflow.com/questions/17988756/how-to-select-lines-between-two-marker-patterns-which-may-occur-multiple-times-w

all: paper-full

paper-full:
	(export TEXINPUTS=${TEXINPUTS};${LATEX} $(FILE); bibtex $(FILE); ${LATEX} $(FILE); ${LATEX} $(FILE))

paper-quick: 
	(export TEXINPUTS=${TEXINPUTS};pdflatex $(FILE))


paper-clean:
	(\rm -rf $(FILE).aux  $(FILE).bbl $(FILE).blg $(FILE).log $(FILE).out  $(FILE).pdf $(FILE).toc texput.log *~)



rep-full:
	(export TEXINPUTS=${TEXINPUTS};${LATEX} $(REP); bibtex $(REP); ${LATEX} $(REP); ${LATEX} $(REP))

rep-quick: 
	(export TEXINPUTS=${TEXINPUTS};pdflatex $(REP))

rep-clean:
	(\rm -rf $(REP).aux  $(REP).bbl $(REP).blg $(REP).log $(REP).out  $(REP).pdf $(REP).toc texput.log *~)



